Determination of Polarization Angles in CMB Experiments and Application to CMB Component Separation Analyses

The new generation of CMB polarization experiments will reach limits of sensitivity never achieved before to detect the primordial B-mode signal. However, all these efforts will be futile if we lack a tight control of systematics. Here, we focus on the systematic that arises from the uncertainty on the calibration of polarization angles. Miscalibrated polarization angles induce a mixing of E- and B-modes that obscures the primordial B-mode signal. We introduce an iterative angular power spectra maximum likelihood-based method to calculate polarization angles from the multi-frequency signal. The basis behind this methodology grounds on nulling the EB power spectra. To simplify the likelihood, we assume that the rotation angles are small (<6 deg) and, the maximum likelihood solution for the rotation angles is obtained by applying an iterative process where the covariance matrix does not depend on the angles per iteration, i.e., the rotation angles are fixed to the estimated angles in the previous iteration. With these assumptions, we obtain an analytical linear system which leads to a very fast computational implementation. We show that with this methodology we are able to determine the rotation angle for each frequency with sufficiently good accuracy. To prove the latter point we perform component separation analyses using the parametric component separation method B-SeCRET with two different approaches. In the first approach we apply the B-SeCRET pipeline to the signal de-rotated with the estimation of the angles, while in the second, the rotation angles are treated as model parameters using the estimation of the angles as a prior information. We obtain that the rotation angles estimations improve after applying the second approach, and show that the systematic residuals due to the non-null calibration polarization angles are mitigated to the order of a 1% at the power spectrum level.

==> impact_on_r.tex <==
Besides, we studied in section~\ref{subsec:cs_impact_on_r} the improvement on the $r$ determination when the rotation angle estimation method is applied using the first approach. The improvement is tested by comparing the component separation results of the following three sets of maps:
\begin{itemize}
    \item \textbf{Non-rotated maps}. The original signal maps without any rotation, i.e., a set of maps without the systematic.
    \item \textbf{Rotated maps}. The previous maps with the corresponding rotation applied, i.e., a set with the systematic.
    \item \textbf{De-rotated maps}. The resulting maps after de-rotating the rotated maps with the solutions obtained with the described methodologies, i.e., a set with the systematic mitigated. This case corresponds to the Approach 1.
\end{itemize}



\subsection{Impact on $r$}
\label{subsec:cs_impact_on_r}

In this section we assess the impact on $r$ of this systematic comparing the results obtained using the approach 1 for each set of maps. In figure~\ref{fig:comparison_non_de_ro_BB_power_spectra} we show the cleaned CMB map $BB$ power-spectra obtained as well as the true residuals\footnote{The true residuals map is calculated as the difference between the cleaned and the input CMB map.} power-spectra, for 4 different simulations. It is evident that the rotated residuals are simulation dependent. Different realizations of the polarization angles introduce systematic errors on the CMB recovery of varying importance. For example, the rotated residuals of simulation 5 are considerably larger than those of simulation 4. On the other hand, we observe that the residuals left in the de-rotated case overlap with the non-rotated's. This means that the proposed method can estimate the leftover polarization angles with sufficient accuracy to remove this systematic effect.
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/qml_bb_power_spectra_comparison_nsim2.pdf}
        \caption{simulation 2}
        \label{subfig:power_spectra_nsim2}
    \end{subfigure}
    \hspace{.01\linewidth}
    \begin{subfigure}{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/qml_bb_power_spectra_comparison_nsim3.pdf}
        \caption{simulation 3}
        \label{subfig:power_spectra_nsim3}
    \end{subfigure}
    \begin{subfigure}{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/qml_bb_power_spectra_comparison_nsim4.pdf}
        \caption{simulation 4}
        \label{subfig:power_spectra_nsim4}
    \end{subfigure}
    \hspace{.01\linewidth}
    \begin{subfigure}{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/qml_bb_power_spectra_comparison_nsim5.pdf}
        \caption{simulation 5}
        \label{subfig:power_spectra_nsim5}
    \end{subfigure}
    \caption{Cleaned CMB (points), residuals (dashed/dashed-dotted lines) and expected, i.e., sum of the CMB model and the residuals, (solid/dotted lines) $BB$ power-spectra of all cases considered, i.e., nonrotated, rotated, de-rotated (red, green and orange colors respectively). The CMB model (lensing) $BB$ power-spectra ($r=0$) is also shown. \bb{no entiendo bien lo que es cada linea. Tambien me parece confuso usar dos tipos de linea (ejemplo solid y dotted) para lo mismo, al menos asi explicado. Creo que es mejor intentar decir mas explicitamente lo que es cada linea. Quiza valdria la pena considerar otros colores para la naranja y la roja que solapan mucho y son colores dificiles de distinguir}}
    \label{fig:comparison_non_de_ro_BB_power_spectra}
\end{figure}
\\
\\
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/qml_observed_minus_residual_model_comparison_nsim1.pdf}
        \caption{simulation 1}
        \label{subfig:difference_power_spectra_nsim1}
    \end{subfigure}
    \hspace{.01\linewidth}
    \begin{subfigure}{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/qml_observed_minus_residual_model_comparison_nsim3.pdf}
        \caption{nsim 3}
        \label{subfig:difference_power_spectra_nsim3}
    \end{subfigure}
    \caption{Difference between the observed and residuals model power-spectrum of all cases considered.}
    \label{fig:comparison_observed_minus_residual}
\end{figure}
\begin{table}
    \centering
    \begin{tabular}{ccccc}
        \toprule
        & \multicolumn{2}{c}{simulation 1} & \multicolumn{2}{c}{simulation 3}  \\
        \midrule
        SET & $\dfrac{r-r^{non}}{\sigma_r^{non}}$ & $\dfrac{\sigma_r}{\sigma_r^{non}}$ & $\dfrac{r-r^{non}}{\sigma_r^{non}}$ & $\dfrac{\sigma_r}{\sigma_r^{non}}$ \\
        \midrule
        Rotated & 15.28 &  1.21 & 32.72 &  1.43 \\ 
        De-rotated & -0.13 & 1.00 & 0.05 &  1.00 \\ 
        \bottomrule
    \end{tabular}
    \caption{$r$ results in the rotated and de-rotated cases compared to the non-rotated case. $\frac{r-r^{non}}{\sigma_r^{non}}$ shows the normalized %\bb{la diferencia relativa suele ser dividiendo por el rnon, quiza decir que es la diferencia normalizada a la dispersion del caso non rotated? } 
    difference with respect to the non-rotated case and $\frac{\sigma_r}{\sigma_r^{non}}$ is the ratio of the uncertainty calculated for a given case with respect to the non-rotated case.} \todo[inline]{\pv{son condicionadas o marginalizadas?} \red{marginalizadas}}
    \label{tab:comparison_r}
\end{table}
\\
\\
We have also evaluated the amount of bias induced in the tensor-to-scalar ratio when the polarization angles are not corrected. Following section 5.1 of \cite{de2020detection} we have obtained an estimation of the residuals left by the component separation approach for each set of maps. Due to the large amount of computational time required to obtain a model of the residuals left after component separation, we have performed this analysis only for two simulations (\bb{\textst{nsim 1 and nsim 3} simulation 1 and 3. Si lo de los residuos se da para la simulacion 1, yo cambiaria alguna de las simulaciones de la figura 13 por la se la simulacion 1, para que este toda la informacion}).  Figure~\ref{fig:comparison_observed_minus_residual} shows the difference between the observed power-spectrum and the estimated residuals model power-spectrum of each set of maps. It is clear that the difference power-spectrum are almost the same in the non-rotated and de-rotated cases while, in the rotated case, we observe that there are some excess residuals compared to the non-rotated case. The procedure that we follow to obtain the residuals models only estimates the amount of foregrounds and noise left after component separation. Thus, the excess in the rotated case is due to systematics related to \bb{\textst{a}} non-null polarization angles.  \\
\\
Furthermore, we have calculated $r$ for each set of maps by fitting the power-spectrum of the cleaned map to the theoretical primordial, the lensing and the residuals model power spectrum \red{using $\chi^2$}. In table~\ref{tab:comparison_r} the results from the rotated and de-rotated cases are compared to the non-rotated case. As expected from figure~\ref{fig:comparison_observed_minus_residual}, the uncertainty on $r$ is the same in the de-rotated and non-rotated case. For the rotated case, the uncertainty on $r$ accounts for the excess residual, hence it is larger than in the non-rotated case. The increase on the uncertainty depends on the systematic introduced on each simulation, i.e., certain combinations of polarization angles results in larger systematic errors than others. On the other hand, we obtain that the $r$ estimation in the de-rotated case is compatible with that of the non-rotated case. However, since the residuals model estimation approach is not able to account for the systematics introduced by polarization angles, the rotated $r$ estimation is non-compatible with the non-rotated estimation. Besides, when polarization angles are not corrected, we can obtain a statistically significant non-null $r$ which is not physical. Hence, the polarization angle correction is essential for the primordial $B$-mode search.  

\bb{si se usa la approach en la que se ajustan los angulos a la vez que los parametros, los residuos tendrian en cuenta errores en la estimacion de los alpha? aunque en este caso parece que es suficiente con ajustar primero los angulos, si el ajuste no fuera tan bueno, quiza seria una forma de tenerlo en cuenta?}

==> old_cross_vs_auto.tex <==
The full formalism presented in section~\ref{sec:methodology} uses the information from all possible combinations of $EB$ cross-spectra. However, the results obtained when all the cross-spectra information is used are significantly worse, especially at the higher frequencies, as it can be seen in figure~\ref{fig:full_auto_cross}.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/full_cross_vs_auto.pdf}
    \caption{Averaged rotation angles over the 100 simulations generated using the information from all possible combinations of $EB$ cross-spectra and only auto-spectra. \pv{por qué se van tanto los puntos azules en el último plot at high-freq?}. \bb{La primera frase es imprecisa, creo que es mejor decir brevemente lo que es cada panel}}
    \label{fig:full_auto_cross}
\end{figure}\\
\\
We have observed that the cause of these incorrect results arises from the use of the observed power spectra \pv{\textst{as the ensemble average} as an estimator for the theoretical} power spectra in the covariance matrix calculation. Specifically, the error comes from a mistaken characterization of the foregrounds' cross-spectra. To demonstrate this claim we have compared the results obtained using the described 100 simulations (figure~\ref{fig:full_auto_cross}) and 100 equivalent simulations without the foreground contributions (figure~\ref{fig:cmb_noise_auto_cross}).
\\
\\
On the other hand, we have studied in this ideal case (only CMB and white noise) the improvement obtained when the full cross-spectra information \pdp{is used} in contrast to \pdp{employing only} the auto-spectra information \pdp{\st{is employed}}. The results are shown in figure~\ref{fig:cmb_noise_auto_cross}. \bb{uniria este parrafo al anterior e incluso al siguiente}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/cmb_noise_cross_vs_auto.pdf}
    \caption{Averaged rotation angles results over 100 simulations of just CMB and noise using the information from all possible combinations of $EB$ cross-spectra and only auto-spectra.\bb{de nuevo describir mejor paneles. Se puede decir que se dan los mismos resultados que en la figura anterior, pero para este otro caso de cmb+ruido}}
    \label{fig:cmb_noise_auto_cross}
\end{figure}
\\
\\
As it was expected, the averaged uncertainty on the rotation angles estimates per channel (see top right panel) are smaller in the cross-spectra case. However, the difference is negligible at the intermediate frequency channels. The larger improvements ($\sim 20$\%) are observed at the most extreme frequencies. The averaged absolute differences between the estimated and the true rotation angles are very similar in both situations \bb{(see top left panel)}. It is clear from the bottom panels that the results are unbiased \bb{esto de nuevo no es del todo correcto} \emg{Yo creo que en este caso puede ser correcto, la mayoría de los casos están entre -0.1-0.1}. The auto\pdp{-spectra} results of $(\alpha_{true}-\alpha_{out})/\sigma_F$ are better mainly because the uncertainties are larger when less information is used. Nonetheless, the cross\pdp{-spectra} results are slightly better when we compare $(\alpha_{true}-\alpha_{out})/\alpha_{true}$ which shows the  deviation from the true estimate fraction. \bb{quiza mejor "the relative error with respect to the true rotation angle"}\\
\\
We conclude that, although \bb{,under ideal conditions,} the results are moderately better when the cross-spectra information is used, the improvement is not critical. Moreover, in section~\ref{sec:component_separation} we prove that the results obtained using only auto-spectra are sufficiently accurate to remove biases due to miscalibrated polarization angles in the $r$ parameter. \\ 
\bb{quiza se puede decir que todos los resultados que se presentan en las siguientes secciones usan solo auto-spectra? (supongo que es asi)}


==> old_methodology.tex <==

Let $N_{ch}$ be the number of frequency channels of the experiment, and $\alpha_{i}$ the $i$-th channel's rotation angle. Assuming a null birefringence angle, the spherical harmonics coefficients of the observed $E$ and $B$ polarization fields of the $i$-th channels are rotated as follows \pv{yo daría alguna ref.}:
\begin{equation}
    \begin{pmatrix}
		E_{i,\ell,m} \\
	    B_{i,\ell,m}
	\end{pmatrix}
	=
	\begin{pmatrix}
		\cos(2\alpha_i) & -\sin(2\alpha_i)\\
	    \sin(2\alpha_i) & \cos(2\alpha_i)\\
	\end{pmatrix}
	\begin{pmatrix}
		E^{*}_{i,\ell,m} \\
	    B^{*}_{i,\ell,m}
	\end{pmatrix} \, ,
	\label{eq:EB_rotated}
\end{equation}
where $E^{*}_{i,\ell,m}$ and $B^{*}_{i,\ell,m}$ are the spherical harmonics coefficients of the non-rotated signal. We define the following auxiliary variables: 
\begin{align}
    \chi_{\ell}^{ij} = \dfrac{C_{\ell}^{E_iB_j} + C_{\ell}^{B_iE_j}}{2}\, , \label{eq:chi_def}\\
    \xi_{\ell}^{ij} = \dfrac{C_{\ell}^{E_iE_j} - C_{\ell}^{B_iB_j}}{2} \, ,  \label{eq:xi_def}
\end{align}
\pdp{aqu\'i el 1/2 en realidad no es necesario} where $C_{\ell}^{X_iY_j} = (2\ell +1)^{-1}\sum_{-m}^{m}X_{i,\ell,m}Y^{*}_{j,\ell,m}$ is the cross power-spectra of  the $X$ and $Y$ fields of the $i$ and $j$ channels respectively.\\
\\
Analogously as in \cite{minami2019simultaneous}, $\chi^{ij}_{\ell}$ can be expressed as
\begin{equation}
    \chi^{ij}_{\ell} = \xi^{ij}_{\ell}\tan\left(2\left(\alpha_i+\alpha_j\right)\right) \, ,
    \label{eq:chi_likelihood_model}
\end{equation}
if we assume that the averaged CMB's and foregrounds' $EB$ cross power-spectra are null \bb{el promedio sobre que?} \pv{se refiere al promedio sobre universos, es decir, que el modelo es cero para CMB y foregrounds. Creo que lo que pasa también es que hay un salto muy grande entre dar los armónicos rotados en función de los armónicos no-rotados, y plantar el likelihood. A lo mejor se puede dar algun apaso intermedio, al estilo del primer paper de Yuto, dando las expresiones de los espectros, e.g., $C_{\ell}^{E_iB_j}$ en función de los ángulos...}. \bb{creo que una buena opcion es dar la derivacion del metodo mas en detalle en un apendice, para que cualquiera lo pueda seguir facilmente. En el otro paper se cita este para los detalles mas tecnicos y creo que es una buena cosa que quede descrito en un articulo para citarlo en el futuro. } Thus, the full log-likelihood (assumed to be Gaussian) of all the possible $EB$-spectra is
\begin{equation}
    -2 \log \mathcal{L} = \sum\limits_{i=1}^{N_{ch}} \sum\limits_{j\geq i}^{N_{ch}} \sum\limits_{i'=1}^{N_{ch}} \sum\limits_{j'\geq i'}^{N_{ch}} \sum\limits_{\ell=\ell_{min}}^{\ell_{max}} \Delta_{\ell}^{ij}(\mymatrix{C}^{-1})_{\ell,ij,i'j'}\Delta_{\ell}^{i'j'}\, ,
    \label{eq:full_likelihood}
\end{equation}
\bb{aunque sea obvio, creo que deberiamos decir que es lmin y lmax}
where $\Delta_{\ell}^{ij} = \chi_{\ell}^{ij} - \xi_{\ell}^{ij}\tan(2\alpha_i + 2\alpha_j)$, and $\mymatrix{C}$ is the  covariance matrix\footnote{It is a $N_{\ell}N_{ch}(N_{ch}+1)/2\times N_{\ell}N_{ch}(N_{ch}+1)/2$ matrix, where $N_{\ell}=\ell_{max}-\ell_{min}$. \pv{no abria que añadil +1 al $N_{\ell}$?}} given as
\begin{align}\label{eq:cov_matrix_cross}
    C_{\ell,ij,i'j'}  = & \dfrac{1}{4\left(2\ell+1\right)}\left\{\left(\ensemble{C}_{\ell}^{E_{i}E_{i'}}\ensemble{C}_{\ell}^{B_{j}B_{j'}} + \ensemble{C}_{\ell}^{E_{i}E_{j'}}\ensemble{C}_{\ell}^{B_{i'}B_{j}} + \ensemble{C}_{\ell}^{B_{i}B_{j'}}\ensemble{C}_{\ell}^{E_{i'}E_{j}} + \ensemble{C}_{\ell}^{B_{i}B_{i'}}\ensemble{C}_{\ell}^{E_{j}E_{j'}} \right.\right. \nonumber\\
    & \left.\left. \ensemble{C}_{\ell}^{E_{i}B_{j'}}\ensemble{C}_{\ell}^{E_{i'}B_{j}} + \ensemble{C}_{\ell}^{E_{i}B_{i'}}\ensemble{C}_{\ell}^{B_{j}E_{j'}} + \ensemble{C}_{\ell}^{B_{i}E_{i'}}\ensemble{C}_{\ell}^{E_{j}B_{j'}} + \ensemble{C}_{\ell}^{B_{i}E_{j'}}\ensemble{C}_{\ell}^{B_{i'}E_{j}} \right)\right. \nonumber\\
    & -c_{i'j'}\left(\ensemble{C}_{\ell}^{E_{i}E_{i'}}\ensemble{C}_{\ell}^{B_{j}E_{j'}} + \ensemble{C}_{\ell}^{E_{i}E_{j'}}\ensemble{C}_{\ell}^{E_{i'}B_{j}} + \ensemble{C}_{\ell}^{B_{i}E_{i'}}\ensemble{C}_{\ell}^{E_{j}E_{j'}} + \ensemble{C}_{\ell}^{B_{i}E_{j'}}\ensemble{C}_{\ell}^{E_{i'}E_{j}}  \right. \nonumber\\
    & \left. -\left(\ensemble{C}_{\ell}^{E_{i}B_{i'}}\ensemble{C}_{\ell}^{B_{j}B_{j'}} + \ensemble{C}_{\ell}^{E_{i}B_{j'}}\ensemble{C}_{\ell}^{B_{i'}B_{j}} + \ensemble{C}_{\ell}^{B_{i}B_{i'}}\ensemble{C}_{\ell}^{E_{j}B_{j'}} + \ensemble{C}_{\ell}^{B_{i}B_{j'}}\ensemble{C}_{\ell}^{B_{i'}E_{j}} \right)\right) \nonumber\\
    & -c_{ij}\left(\ensemble{C}_{\ell}^{E_{i}E_{i'}}\ensemble{C}_{\ell}^{E_{j}B_{j'}} + \ensemble{C}_{\ell}^{E_{i}B_{j'}}\ensemble{C}_{\ell}^{E_{i'}E_{j}} + \ensemble{C}_{\ell}^{E_{i}B_{i'}}\ensemble{C}_{\ell}^{E_{j}E_{j'}} + \ensemble{C}_{\ell}^{E_{i}E_{j'}}\ensemble{C}_{\ell}^{B_{i'}E_{j}}  \right. \nonumber\\
    & \left. -\left(\ensemble{C}_{\ell}^{B_{i}E_{i'}}\ensemble{C}_{\ell}^{B_{j}B_{j'}} + \ensemble{C}_{\ell}^{B_{i}B_{j'}}\ensemble{C}_{\ell}^{E_{i'}B_{j}} + \ensemble{C}_{\ell}^{B_{i}B_{i'}}\ensemble{C}_{\ell}^{B_{j}E_{j'}} + \ensemble{C}_{\ell}^{B_{i}E_{j'}}\ensemble{C}_{\ell}^{B_{i'}B_{j}} \right)\right) \nonumber\\
    & -c_{i'j'}c_{ij}\left(\ensemble{C}_{\ell}^{E_{i}E_{i'}}\ensemble{C}_{\ell}^{E_{j}E_{j'}} + \ensemble{C}_{\ell}^{E_{i}E_{j'}}\ensemble{C}_{\ell}^{E_{i'}E_{j}} + \ensemble{C}_{\ell}^{B_{i}B_{i'}}\ensemble{C}_{\ell}^{B_{j}B_{j'}} + \ensemble{C}_{\ell}^{B_{i}B_{j'}}\ensemble{C}_{\ell}^{B_{i'}B_{j}}  \right. \nonumber\\
    & \left.\left. -\left(\ensemble{C}_{\ell}^{E_{i}B_{i'}}\ensemble{C}_{\ell}^{E_{j}B_{j'}} + \ensemble{C}_{\ell}^{E_{i}B_{j'}}\ensemble{C}_{\ell}^{B_{i'}E_{j}} + \ensemble{C}_{\ell}^{B_{i}E_{i'}}\ensemble{C}_{\ell}^{B_{j}E_{j'}} + \ensemble{C}_{\ell}^{B_{i}E_{j'}}\ensemble{C}_{\ell}^{E_{i'}B_{j}} \right)\right) \right\} \, ,\nonumber\\
\end{align}
\pdp{ Creo que deber\'ia ser $c_{i'j'}c_{ij}$ en vez de -$c_{i'j'}c_{ij}$. Tambi\'en estamos despreciando las correlaciones $\ell\times\ell'$} where $c_{kl} = \tan\left(2\left(\alpha_{k}+\alpha_{l}\right)\right)$, and  $\ensemble{C}_{\ell}^{XY}$ is the ensemble average of the $XY$ power-spectrum. Due to the lack of a reliable model of the foregrounds cross-spectra, we require a good estimator of it from the observed power-spectra. In section~\ref{subsec:covariance_matrix_model} we will study several estimators and will show that binning the observed power-spectrum leads to competent results.\\
\\
Assuming: \bb{como no se enlaza la frase despues de los items, parece que la frase esta incompleta, sugiero "Let us assume:"}
\begin{itemize}
    \item Small angle approximation: $\alpha \ll 1 \rightarrow \tan(\alpha) \sim \alpha$.
    \item The covariance matrix $\mymatrix{C}$ does not depend on $\alpha$. To circumvent the mismatch induced by this approximation, we perform an iterative approach that updates the polarization angle in the covariance matrix with the one estimated in the previous step. \pv{A lo mejor aquí también se podría enlazar con la discusión de los papers que mencionó Komatsu en la telecon de NPIPE, en el sentido de que, en realidad, es mejor no hacer depender la matriz de covarianza de los parámetros, a la hora de estimarlos...}
\end{itemize} 
With these approximations, we achieve a linear system which enables us to obtain analytical equations from \ref{eq:full_likelihood} to calculate the rotation angles. Moreover, the uncertainties can be evaluated from the Fisher matrix. This results in a very fast computational methodology.  \\
\\
Although the formalism exposed uses the information from cross-spectra among all channels, one can  limit the information to only auto-spectra (i.e., no correlation among different channels) $EB$-spectra. In this case, with all the approximations made, the likelihood simplifies to 
\begin{equation}
    -2 \log \mathcal{L} = \sum\limits_{i=1}^{N_{ch}}  \sum\limits_{j=1}^{N_{ch}}  \sum\limits_{\ell=\ell_{min}}^{\ell_{max}} \left(C_{\ell}^{E_iB_i} - 4\alpha_i\xi_{\ell}^{ii}\right)\left(\mymatrix{C}^{-1}\right)_{\ell,ij}
    \left(C_{\ell}^{E_jB_j} - 4\alpha_j\xi_{\ell}^{jj}\right)\, ,
    \label{eq:auto_likelihood}
\end{equation}
and the covariance matrix is 
\begin{align}
    C_{\ell,i,j} = \dfrac{1}{2\ell +1} 
     & \left(\left(\ensemble{C}_{\ell}^{E_iE_j,o}\ensemble{C}_{\ell}^{B_iB_j,o} + \ensemble{C}_{\ell}^{E_iB_j,o}\ensemble{C}_{\ell}^{B_iE_j,o} \right)\right.\nonumber \\  
     & - 4\alpha_j\left(\ensemble{C}_{\ell}^{E_iE_j,o}\ensemble{C}_{\ell}^{B_iE_j,o} - \ensemble{C}_{\ell}^{E_iB_j,o}\ensemble{C}_{\ell}^{B_iB_j,o}\right) \nonumber \\
    & - 4\alpha_i\left(\ensemble{C}_{\ell}^{E_iE_j,o}\ensemble{C}_{\ell}^{E_iB_j,o} - \ensemble{C}_{\ell}^{B_iE_j,o}\ensemble{C}_{\ell}^{B_iB_j,o}\right) \nonumber\\
    & \left . + 8\alpha_i\alpha_j\left(\left(\ensemble{C}_{\ell}^{E_iE_j,o}\right)^2 + \left(\ensemble{C}_{\ell}^{B_iB_j,o}\right)^2 -\left(\ensemble{C}_{\ell}^{E_iB_j,o}\right)^2 + \left(\ensemble{C}_{\ell}^{B_iE_j,o}\right)^2 \right)\right)  \, .
    \label{eq:auto_covariance_matrix}
\end{align}
\pdp{mantenemos las tangentes en el cálculo de la matriz de covarianza o aplicamos la aproximaci\'on de \'angulos pequeños?}\red{tengo las dos implementaciones y funcionan igual en principio he puesto con aproximaci\'on} Owing to the use of an estimator of the emsemble average power-spectra in the covariance matrix calculation instead of the true model, we have seen that results are biased when all the cross power-spectra information is used (see section \ref{subsec:cross_cmbnoise}). Therefore, in this work we use only the auto spectra.\pv{No sé si se le puede dar una mejor salida a esto, por ejemplo en NPIPE lo estamos intentado usar. A lo mejor decir que cuando estamos dominados por ruido, se pueden meter?} \\
\\
The rotation angles are obtained after solving the following linear system obtained from eq. \ref{eq:auto_likelihood} \pv{decir un poc más. en el sentido de que derivamos con respecto a los parámetros e igualamos a cero, para el contrar el maximum-likelihood?}:
\begin{equation}
    \mymatrix{\Omega}\myvector{\alpha} = \dfrac{1}{4}\myvector{\eta} \, , \label{eq:auto_angles_linear_system}
\end{equation}
where $\mymatrix{\Omega}$ \pv{matrix }and $\myvector{\eta}$ \pv{vector have the following} elements \pv{\textst{are}}:
\begin{align}
    \Omega_{ij} = \sum\limits_{\ell=\ell_{min}}^{\ell_{max}} \xi_{\ell}^{ii}\left(\mymatrix{C}^{-1}\right)_{\ell,ij}\xi_{\ell}^{jj} \, , 
    \label{eq:omega_element} \\
    \eta_{i} = \sum\limits_{j=1}^{N_{ch}}\sum\limits_{\ell=\ell_{min}}^{\ell_{max}} \xi_{\ell}^{ii}\left(\mymatrix{C}^{-1}\right)_{\ell,ij}C_{\ell}^{E_jB_j} \, .
    \label{eq:eta_element}
  \end{align} 
The rotation angles' uncertainties are obtained from the Fisher matrix \cite{coe2009fisher}, whose elements are given as
\begin{equation}
    F_{ij} = \dfrac{1}{2}\dfrac{\partial^2 (-2\log \mathcal{L})}{\partial \alpha_{i}\partial \alpha_{j}} = 16 \sum\limits_{\ell=\ell_{min}}^{\ell_{max}} \xi_{\ell}^{ii}\left(\mymatrix{C}^{-1}\right)_{\ell,ij}\xi_{\ell}^{jj}\, .
    \label{eq:Fisher_auto_elements}
\end{equation}

